ARC: Fair Relative Advantage Comparison in Open-Ended Real-World Interaction

Open-ended real-world interaction admits multiple valid behaviors: an agent may answer directly, ask for clarification, provide progress updates, or confirm before acting. This flexibility breaks a core assumption behind group-based RL: rollouts compared within a group are no longer guaranteed to be behaviorally comparable. As a result, reward-model preferences over interaction style can distort relative advantages and steer optimization toward reward-preferred behaviors rather than context-appropriate ones. We formalize this as a \textit{reward fairness problem} and propose \textbf{ARC} (Advantage Regularization via Conditioning), a training recipe that restores fairer relative comparison through strategy-conditioned rollout grouping, together with hybrid rewards and entropy regularization. We study ARC in our proposed \inter, a novel paradigm for responsive, steerable, and execution-aware user-agent interaction that decouples user-visible communication from latent reasoning and tool use. \inter\ also provides the annotation and distillation pipeline for constructing \inter-86K, our strategy-annotated training corpus for supervised and RL training. Empirically, ARC substantially strengthens the core $\tau/\tau^2$ tool-use benchmarks, while \inter\ reduces time-to-first-token from 4.91s to 1.27s relative to a think-style baseline. Together, these results suggest that a central bottleneck in open-ended interactive learning is not only how agents are rewarded, but whether their behaviors are compared fairly in the first place. The ARC implementation and \inter-86K training data will be released.

==> macros.tex <==
% Project-specific notation belongs here.
% Keep macros semantic and avoid styling commands in manuscript prose.
\newcommand{\model}{\textsc{ExampleModel}}
\newcommand{\dataset}{\textsc{ExampleBench}}
\newcommand{\method}{\textsc{ExampleMethod}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}



==> sections/01-introduction.tex <==
\section{Introduction}

Open with the concrete capability, evaluation, or deployment goal that the
paper accepts. Then identify the same-axis condition under which the existing
route becomes unreliable, expensive, or incomplete. Avoid broad field-history
openings that delay the paper's actual proof obligation.

State the revised success criterion before introducing the system name. Each
principal component should answer a constraint already made visible to the
reader. Prior work belongs where it licenses the motivation or contrast, not
only in a detached related-work section \citep{vaswani2017attention}.

\AntKeyPoint{%
  A strong introduction creates method necessity before it inventories
  components: shared goal $\rightarrow$ precise tension $\rightarrow$ success
  criterion $\rightarrow$ constraint-derived method $\rightarrow$ signature
  evidence.
}

\paragraph{Contributions.}
Use two to four non-overlapping contributions. Each item should state what new
knowledge or capability is provided and point to the evidence that supports it.
\begin{itemize}
  \item A precise problem or construct that makes the missing distinction
        measurable.
  \item A method or resource whose components follow from the stated
        constraints.
  \item An evaluation that repays the paper's central promises and exposes its
        failure boundary.
\end{itemize}



==> sections/02-method.tex <==
\section{Method}

Define paper-specific objects before drawing conclusions from them. For each
core component, explain the failure it addresses, the resulting design
criterion, the mechanism, and the expected effect.

\subsection{Problem Formulation}

Let $x \in \mathcal{X}$ denote an input and $y \in \mathcal{Y}$ a target. A
minimal objective can be written as
\begin{equation}
  \theta^\star =
  \arg\min_{\theta \in \R^d}
  \E_{(x,y)\sim\mathcal{D}}
  \left[\mathcal{L}\bigl(f_\theta(x),y\bigr)\right].
  \label{eq:objective}
\end{equation}
Retain only notation that supports later reasoning, an experimental variable,
or an otherwise ambiguous definition.

\subsection{System Design}

Use a wide figure only when the comparison or architecture genuinely benefits
from the full page width.

\begin{figure*}[t]
  \begin{tcolorbox}[
    enhanced,
    colback=white,
    colframe=AntRule,
    boxrule=0.6pt,
    arc=2mm,
    left=4mm,right=4mm,top=4mm,bottom=4mm]
    \begin{minipage}[c]{0.28\textwidth}
      \centering\sffamily\bfseries\color{black}
      1. Grounded Input\\[-1pt]
      {\footnotesize\mdseries\color{black}Data, context, and constraints}
    \end{minipage}
    \hfill{\Large\color{AntBright}$\longrightarrow$}\hfill
    \begin{minipage}[c]{0.28\textwidth}
      \centering\sffamily\bfseries\color{black}
      2. Verifiable Process\\[-1pt]
      {\footnotesize\mdseries\color{black}Method, checks, and controls}
    \end{minipage}
    \hfill{\Large\color{AntBright}$\longrightarrow$}\hfill
    \begin{minipage}[c]{0.28\textwidth}
      \centering\sffamily\bfseries\color{black}
      3. Measured Outcome\\[-1pt]
      {\footnotesize\mdseries\color{black}Evidence and failure boundary}
    \end{minipage}
  \end{tcolorbox}
  \caption{Example full-width system overview. The caption identifies the
  comparison and defines the visual grammar; the main text should explain why
  the relationship matters.}
  \label{fig:overview}
\end{figure*}


==> sections/03-experiments.tex <==
\section{Experiments}

Introduce the experimental question before the table or figure used to answer
it. Specify what changes, what is held fixed, the evaluated population, the
metric, the pairing unit, and the uncertainty procedure.

\subsection{Main Results}

Table~\ref{tab:main} demonstrates the default table grammar. Use bold only for
the comparison that matters; do not turn every local maximum into visual noise.

\begin{table}[t]
  \caption{Example results under a shared evaluation protocol. Higher is
  better for both metrics. Replace all values with audited results.}
  \label{tab:main}
  \centering
  \begin{tabular}{lcc}
    \toprule
    Method & Primary (\%) & Robustness (\%) \\
    \midrule
    Baseline A & 71.2 & 63.5 \\
    Baseline B & 73.8 & 66.1 \\
    \method{}  & \textbf{77.4} & \textbf{70.8} \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Observation.}
State what the evidence directly shows.
\paragraph{Interpretation.}
Explain why the pattern may arise and distinguish measured support from a
plausible mechanism.
\paragraph{Boundary.}
Name the setting, population, or intervention outside which the conclusion is
not established.

\subsection{Ablations and Failure Analysis}

An ablation should test design necessity, not merely show that removing a large
fraction of the system lowers performance. Pair aggregate results with
representative failures when they expose a distinct limitation.



==> sections/04-discussion.tex <==
\section{Discussion and Limitations}

Anchor the discussion in the minimum empirical finding needed for the
interpretation. Then state the nearest research or deployment decision that
changes if the finding holds.

Limitations should narrow named claims. Identify the evidence, control, or
design change needed to remove each boundary. Do not use this section as a
generic list of future directions.



==> sections/05-conclusion.tex <==
\section{Conclusion}

Close the supported thesis without introducing a new contribution. A useful
conclusion reconnects the problem, the paper's intervention, the signature
evidence, and the exact scope of the resulting implication.


